On Bundle Adjustment for Multiview PointCloud Registration

Multiview registration is used to estimate Rigid Body Transformations (RBTs) from multiple frames and reconstruct a scene with corresponding scans. Despite the success of pairwise registration and pose synchronization, the concept of Bundle Adjustment (BA) has been proven to better maintain global consistency. So in this work, we make the multiview point-cloud registration more tractable from a different perspective in resolving range-based BA. Based on this analysis, we propose an objective function that takes both measurement noises and computational cost into account. For the feature parameter update, instead of calculating the global distribution parameters from the raw measurements, we aggregate the local distributions upon the pose update at each iteration. The computational cost of feature update is then only dependent on the number of scans. Finally, we develop a multiview registration system using voxel-based quantization that can be applied in real-world scenarios. The experimental results demonstrate our superiority over the baselines in terms of both accuracy and speed. Moreover, the results also show that our average positioning errors achieve the centimeter level.

==> conclusion.tex <==
\section{Conclusions and Future Work}
\label{sec:conclusions}

% STEP. long
% In this paper, we presented a monocular VO system leveraging deep description and repeatability.
% % We discuss
% % Different from previous work, we focus on explore a better way to.
% Not only extract the local features from the predicted repeatability, we further parameterize them as 2-D Gaussian component to model the uncertainty of prediction.
% Then, we propose a direct tracking scheme to estimate the camera pose coarsely.
% Afterwards, patch-wise association can be performed efficiently by check the inliers with neibourhoods.
% % To generate correspondences for triangualtion
% The experimetal results demonstrate the proposed system is capable to handle challenging situation, where both the state-of-the-art indirect and direct methods suffer from strong degradation.
% For the rumtime analysis, as the proposed system maintain a more lightweight backend than ORB-SLAM, the computation time of typical modules is dramatically reduced despite the feature extraction frontend.
% In the future, we would like to investigate supervising the feature detection and description frontend in an end-to-end manner.
% Introducing geometric constraints might benefits the learning process.

% STEP. short 
% TODO: rewrite
In this paper, we presented a monocular VO system leveraging learned description and repeatability.
% We discuss
Different from previous work, we focused on tightly coupling the learning-based frontend with indirect multiview geometry to fully exploit the network predictions.
% To achieve this goal, 
% the parameterization of local feature is discussed
% Not only extract the local features from the predicted repeatability, we further parameterize them as 2-D Gaussian component to model the uncertainty of prediction.
% To achieve this goal, we first extract local salient point
We proposed a two-step tracking scheme to estimate the camera pose: direct tracking on the repeatability maps and refining the pose with the patch-wise association.
The adapted mapping module maintained a lightweight and consistent backend.
% ANN along with grid-search on epipolar line associated features for triangualtion, with which a lightweight and consistent backend was maintained.
% Epipolar line search 
% Adapted mapping module 
% For the consideration of unc
% Adapted mapping module 
% The local feature parameterization was discussed to model the uncertainty.
% Grid search along epipolar line 
% Different mapping methods were discussed and adopted into the systematic implementation.
% Local feature parameterization 
%  coarsely.
% Afterwards, patch-wise association can be performed efficiently by check the inliers with neibourhoods.
% To generate correspondences for triangualtion
The experimental results demonstrated that the proposed system is capable to handle challenging situations, where both the state-of-the-art indirect and direct methods suffer from strong degradation.
% For the runtime analysis, as the proposed system maintain a more lightweight backend than ORB-SLAM, the computation time of typical modules is dramatically reduced despite the feature extraction frontend.
In the future, we would like to investigate supervising the feature detection and description frontend in an end-to-end manner and improving the network prediction speed for onboard visual state estimation.

    


